Machine learning metallic glass critical cooling rates through elemental and molecular simulation based featurization

We have developed a machine learning model for critical cooling rates for metallic glasses based on computational properties. We compare results for features derived from easy-to-compute functions of elemental properties to more complex physically motivated properties using ab initio, machine-learning potentials, and empirical potential molecular dynamics methods. The established approach enables property acquisition across a diverse range of alloys. Analysis of various features for 34 alloys from 20 chemical systems shows that the best model for critical cooling rates was learned from one elemental property-based feature and three simulated features. The elemental property-based feature is an ideal entropy value based on alloy stoichiometry. The simulated features were acquired from estimates of energies above the convex hull, changes in heat capacity, and the fraction of icosahedra-like Voronoi polyhedra. Models were assessed through a demanding cross validation test based on repeatedly leaving out full chemical systems as test sets and had an $R^2$ of 0.78 and a mean average error of 0.76 in units of $[log_{10}(K/s)]$. We demonstrate with Shapley additive explanation analysis that the most impactful features have physically reasonable influence on model predictions. The established methodology can be applied to other high-throughput studies of material properties of diverse compositions.

==> tables/mtp_sizes.tex <==
\begin{table}[H]
\centering
\caption{The training set size for MTPs are shown.}
\label{mtp_train_sizes}
\begin{tabular}{lr}
\toprule
          Composition &  Size \\
\midrule
Nb7Ni59Si3Sn2Ti13Zr16 &  2541 \\
   Al25Co5Cu10La55Ni5 &  1773 \\
 Be25Cu10Ni10Ti11Zr44 &  1510 \\
      Al8Cu12Ni14Zr66 &  1255 \\
      Al25Cu5La55Ni15 &  1247 \\
     Al25Cu10La55Ni10 &  1230 \\
       Al9Cu16Ni9Zr66 &  1223 \\
       Al8Cu7Ni19Zr66 &  1203 \\
      Al25Cu15La55Ni5 &  1195 \\
      Cu25Ni10P20Pd45 &  1173 \\
      Cu25Ni15P20Pd40 &  1172 \\
      Cu30Ni10P20Pd40 &  1160 \\
         Ca65Mg15Zn20 &  1081 \\
      Cu47Ni8Ti34Zr11 &  1066 \\
       Cu30Ni5P20Pd45 &  1046 \\
          Ni40P20Pd40 &  1039 \\
         Al25Cu20La55 &  1020 \\
         Al14Cu20La66 &  1011 \\
         Mg65Nd15Ni20 &  1010 \\
         Mg70Nd15Ni15 &  1003 \\
           Mg90Nd5Ni5 &   992 \\
          Mg77Nd5Ni18 &   990 \\
         Mg75Nd10Ni15 &   978 \\
         Mg80Nd10Ni10 &   978 \\
         Al25La55Ni20 &   955 \\
          Al8Ni26Zr66 &   946 \\
          Cu6Pd77Si17 &   917 \\
             Be37Ti63 &   903 \\
              Pd95Si5 &   893 \\
         Cu25Gd10Mg65 &   889 \\
          Cu25Mg65Y10 &   889 \\
             Pd82Si18 &   881 \\
             Be35Zr65 &   870 \\
             Pd75Si25 &   870 \\
             Nb40Ni60 &   861 \\
\bottomrule
\end{tabular}
\end{table}

